Can You Explain That, Better? Comprehensible Text Analytics for SE Applications

Text mining methods are used for a wide range of Software Engineering (SE) tasks. The biggest challenge of text mining is high dimensional data, i.e., a corpus of documents can contain $10^4$ to $10^6$ unique words. To address this complexity, some very convoluted text mining methods have been applied. Is that complexity necessary? Are there simpler ways to quickly generate models that perform as well as the more convoluted methods and also be human-readable? To answer these questions, we explore a combination of LDA (Latent Dirichlet Allocation) and FFTs (Fast and Frugal Trees) to classify NASA software bug reports from six different projects. Designed using principles from psychological science, FFTs return very small models that are human-comprehensible. When compared to the commonly used text mining method and a recent state-of-the-art-system (search-based SE method that automatically tune the control parameters of LDA), these FFT models are very small (a binary tree of depth $d = 4$ that references only 4 topics) and hence easy to understand. They were also faster to generate and produced similar or better severity predictions. Hence we can conclude that, at least for datasets explored here, convoluted text mining models can be deprecated in favor of simpler method such as LDA+FFTs. At the very least, we recommend LDA+FFTs (a) when humans need to read, understand, and audit a model or (b) as an initial baseline method for the SE researchers exploring text artifacts from software projects.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


***************************** Subdirectories ******************************

bibtex   - The IEEEtran BibTeX style package.

extras   - Supplementary material that may be of interest.

testflow - The testflow diagnostic suite for verifying PS/PDF output.

tools    - The IEEEtrantools.sty package which provides several commands
           from the IEEEtran.cls file for use with other LaTeX classes.


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex,
                   bare_jrnl.tex, bare_jrnl_comsoc.tex,
                   bare_jrnl_compsoc.tex, bare_jrnl_transmag.tex
***************************************************************************


==> figs/interpretability.tex <==
\makeatletter
\newcommand{\verbatimfont}[1]{\def\verbatim@font{#1}}%
\makeatother
\verbatimfont{\times}


\begin{figure*}[!t]
 {\small

\begin{minipage}{\linewidth}
\begin{lstlisting}[
  mathescape,
  columns=fullflexible,
  basicstyle=\fontfamily{times}\selectfont,
]
                                               PITS_A Dataset
if topic 1 >  0.8 then false  Topic 1: type data line code statu packet word function
      else if topic 7 >  0.6     then true \hspace{0.5cm}                      Topic 7: mode point control project attitud rate error prd
      else if topic 3 >  0.65    then true                      Topic 3: messag unsign bit code file byte word ptr
      else if topic 5 =< 0.5     then true                      Topic 5: file variabl code symbol messag line initi access 
      else false 
\end{lstlisting}


  \end{minipage}
%\end{flushright}
\begin{minipage}{\linewidth}
\begin{verbatim}
                                               PITS_B Dataset
      if      topic 2 >  0.7     then true                     Topic 2: command gce counter step bgi test state antenna
      else if topic 4 >  0.75    then false                    Topic 4: line code function file declar comment return use
      else if topic 7 >  0.65    then true                     Topic 7: ace command fsw shall level state trace packet
      else if topic 6 =< 0.8     then true                     Topic 6: test interfac plan file dmr document section data 
      else false 
  \end{verbatim}
  \end{minipage}
  
\begin{minipage}{\linewidth}
\begin{verbatim}
                                               PITS_C Dataset
      if      topic 1 >  0.7     then false                    Topic 1: requir fsw command specif state specifi shall ground
      else if topic 6 >  0.55    then true                     Topic 6: tim trace section document traceabl matrix rqt requir
      else if topic 8 >  0.73    then true                     Topic 8: appropri thermal field integr test valid ram violat
      else if topic 2 >  0.85    then false                    Topic 2: header zero posit network indic action spacecraft base
      else true 
\end{verbatim}\end{minipage}
  
\begin{minipage}{\linewidth}
\begin{verbatim}
                                               PITS_D Dataset
      if      topic 6 <= 0.5     then false                    Topic 6: essenti record heater occurr indic includ rollov  
      else if topic 1 >  0.8     then true                     Topic 1: fsw csc trace data field fpa tabl command
      else if topic 4 >  0.85    then false                    Topic 4: enabl wheel use disabl respons control protect fault
      else if topic 9 >  0.6     then false                    Topic 9: line cpp case switch default projectd file fsw
      else true 
\end{verbatim}\end{minipage}
  
  
\begin{minipage}{\linewidth}
\begin{verbatim}
                                               PITS_E Dataset
      if      topic 8  > 0.75    then true                     Topic 8: line file function cmd paramet ccu fsw vml
      else if topic 5  > 0.7     then false                    Topic 5: inst phx test project set document softwar verifi
      else if topic 7  > 0.5     then false                    Topic 7: ptr size time prioriti ega defin data null
      else if topic 10 < 0.9     then false                    Topic 10: word fsw enabl capabl follow vagu present emic
      else true 
  \end{verbatim}
  \end{minipage}
\begin{minipage}{\linewidth}
\begin{verbatim}
                                               PITS_F Dataset
      if      topic 5 <= 0.8     then false                    Topic 4: requir projectf tabl ref boot bsw fsw section
      else if topic 8  > 0.75    then true                     Topic 7: fsw requir test projectf procedur suffici softwar 
      else if topic 2  > 0.5     then true                     Topic 1: code variabl test point build defin float valu 
      else if topic 9  > 0.65    then true                     Topic 8: number byte word limit buffer dump ffp error 
      else false 
  \end{verbatim}
  \end{minipage}
}
\caption{Comprehensible models generated by FFT for all 6 datasets }
\label{fig:comprehensible}
\end{figure*}

==> figs/interpretability_2.tex <==
\begin{figure*}[!t]
 {\scriptsize

\begin{minipage}{\linewidth}
\begin{verbatim}
                                               PITS_A Dataset
      if      topic 1 >  0.8     then false                    Topic 1: type data line code statu packet word function
      else if topic 7 >  0.6     then true                     Topic 7: mode point control project attitud rate error prd
      else if topic 3 >  0.65    then true                     Topic 3: messag unsign bit code file byte word ptr
      else if topic 5 =< 0.5     then true                     Topic 5: file variabl code symbol messag line initi access 
      else false 
  \end{verbatim}
  \end{minipage}
%\end{flushright}
\begin{minipage}{\linewidth}
\begin{verbatim}
                                               PITS_B Dataset
      if      topic 2 >  0.7     then true                     Topic 2: command gce counter step bgi test state antenna
      else if topic 4 >  0.75    then false                    Topic 4: line code function file declar comment return use
      else if topic 7 >  0.65    then true                     Topic 7: ace command fsw shall level state trace packet
      else if topic 6 =< 0.8     then true                     Topic 6: test interfac plan file dmr document section data 
      else false 
  \end{verbatim}
  \end{minipage}
  
\begin{minipage}{\linewidth}
\begin{verbatim}
                                               PITS_C Dataset
      if      topic 1 >  0.7     then false                    Topic 1: requir fsw command specif state specifi shall ground
      else if topic 6 >  0.55    then true                     Topic 6: tim trace section document traceabl matrix rqt requir
      else if topic 8 >  0.73    then true                     Topic 8: appropri thermal field integr test valid ram violat
      else if topic 2 >  0.85    then false                    Topic 2: header zero posit network indic action spacecraft base
      else true 
\end{verbatim}\end{minipage}
  
\begin{minipage}{\linewidth}
\begin{verbatim}
                                               PITS_D Dataset
      if      topic 6 <= 0.5     then false                    Topic 6: essenti record heater occurr indic includ rollov  
      else if topic 1 >  0.8     then true                     Topic 1: fsw csc trace data field fpa tabl command
      else if topic 4 >  0.85    then false                    Topic 4: enabl wheel use disabl respons control protect fault
      else if topic 9 >  0.6     then false                    Topic 9: line cpp case switch default projectd file fsw
      else true 
\end{verbatim}\end{minipage}
  
  
\begin{minipage}{\linewidth}
\begin{verbatim}
                                               PITS_E Dataset
      if      topic 8  > 0.75    then true                     Topic 8: line file function cmd paramet ccu fsw vml
      else if topic 5  > 0.7     then false                    Topic 5: inst phx test project set document softwar verifi
      else if topic 7  > 0.5     then false                    Topic 7: ptr size time prioriti ega defin data null
      else if topic 10 < 0.9     then false                    Topic 10: word fsw enabl capabl follow vagu present emic
      else true 
  \end{verbatim}
  \end{minipage}
\begin{minipage}{\linewidth}
\begin{verbatim}
                                               PITS_F Dataset
      if      topic 5 <= 0.8     then false                    Topic 4: requir projectf tabl ref boot bsw fsw section
      else if topic 8  > 0.75    then true                     Topic 7: fsw requir test projectf procedur suffici softwar 
      else if topic 2  > 0.5     then true                     Topic 1: code variabl test point build defin float valu 
      else if topic 9  > 0.65    then true                     Topic 8: number byte word limit buffer dump ffp error 
      else false 
  \end{verbatim}
  \end{minipage}
}
\caption{Comprehensible models generated by FFT for all 6 datasets }
\label{fig:comprehensible}
\end{figure*}

==> figs/raw.tex <==
\iffalse

The most common text mining technique for binary classification in software engineering is TFIDF as the feature extraction method with SVM as a classifier. 
In recent studies~\cite{agrawal2018wrong,layman2016topic}, LDA feature extraction is shown to be a great alternative due to it achieving similar performance as well reduction in dimensionality. 
LDA features also provide better sense of interpretability only if we have 10s of features not 100s. FFT is shown to be a good classifier when dealing with low dimensionality~\cite{fu2018building,chen2018applications}. That is why we compared TFIDF+SVM against LDA+FFT. We tried multiple combinations of LDA features like ($K=10, 25, 50, 100$) with its other default values.

Figure~\ref{fig:} offers a statistical analysis of different results achieved between TFIDF+SVM, LDADE+SVM, LDA+FFT against 10\_FFT, 25\_FFT, 50\_FFT, 100\_FFT. X-axis is the figure represents different datasets and Y-axis represents precision and recall scores.    For any learner, there are median and IQR range being recorded, the \textit{darker} the cell, the \textit{better} the performance. In the figure the same color are either not statistically significant or are different only via a \textit{small} effect (as stated by the statistical methods described in Section  \ref{sec:scott-knott}).  
 
\subsection*{\textbf{RQ1: {\em How does simpler method \textit{perform} against most common convoluted methods and recent state of the art search based SE method?} }}

The most common text mining technique for binary classification in software engineering is TFIDF as the feature extraction method with SVM as a classifier. In recent studies~\cite{agrawal2018wrong,layman2016topic}, LDA feature extraction is shown to be a great alternative due to it achieving similar performance as well reduction in dimensionality. 

At the same time, a lot of researchers have adapted hyperparamete tuning to optimize performance but they do come with an expense of heavy runtime~\cite{fu2016tuning,ghotra2015revisiting,agrawal2018wrong,agrawal2018better}. Agrawal et al.~\cite{agrawal2018wrong} showed LDADE to achieve better performance in classification task with SVM as a classifier. LDADE chooses optimal $K$, $\alpha$ and $\beta$, but $K$ matters the most for supervised learning.

LDA features also provide better sense of interpretability only if we have 10s of features not 100s. FFT is shown to be a good classifier when dealing with low dimensionality~\cite{fu2018building,chen2018applications}. That is why we compared TFIDF+SVM against LDA+FFT. We tried multiple combinations of LDA features like ($K=10, 25, 50, 100$) with its other default values. In this research question, we compared TFIDF+SVM as our picked convoluted methods and LDADE+SVM, LDADE+FFT as recent state of the art search based SE method against LDA+FFT. We tried multiple combinations of LDA features like ($K=10, 25, 50, 100$) with its other default values.

For recall, from Figure \ref{fig:} we can observe that 10\_FFT, 25\_FFT, 50\_FFT, 100\_FFT are performing statistically similar against all 6 datasets. At the same time, out of 6 datasets, they are statistically winning against TFIDF+SVM on 3, losing on 1, and are providing statistically similar results on the remaining 2 datasets. Since all $K$ values are performing similarly, we can choose $K=10$ as the optimal number of features that are needed for the FFT model.

For precision, a similar trend was observed where 10\_FFT, 25\_FFT, 50\_FFT, 100\_FFT are performing statistically similar (4 out of 6 datasets) but TFIDF+SVM is winning statistically 3 out of 6 datasets and is performing similar on the remaining 3 datasets. Since all $K$ values are performing similarly and with $K=10$, the model wins twice out of six, $K=10$ will be picked as the optimal number of features that are needed.

With any empirical study, beside performance, we have to look at the runtimes as another criteria to evaluate the models to make sure that the advantage do not come at a cost of a large runtime. Table~\ref{tbl:runtimes} shows the runtimes in minutes. From the table, it can be observed that LDA+FFT combination is about 100 times slower than TFIDF+SVM. If we have a business case where researchers/engineers need to interpret the model then the trade-off between the runtime and interpretability is not large.




% \begin{figure}[!t]
%         \centering
%         \includegraphics[width=\linewidth]{./figs/graph2.png}

%     \caption{ Comparison of FFT with SVM TFIDF }
%     \label{fig:rq1}
% \end{figure}

For Interpretability

% \begin{table*}[!t]
% \centering
% \caption{Runtimes (in minutes)}
% \label{tbl:runtimes}
% \begin{tabular}{c|c|c|c|c|c|c|c}

%                                      & \textbf{TFIDF\_SVM} & \textbf{10\_FFT} & \textbf{25\_FFT} & \textbf{50\_FFT} & \textbf{100\_FFT} & \textbf{LDADE\_FFT} & \textbf{LDADE\_SVM} \\ \hline
% \multicolumn{1}{l|}{\textbf{PitsA}} & <1                   & 431              & 519              & 715              & 1381              & 49422               & 49395               \\ \hline
% \multicolumn{1}{l|}{\textbf{PitsB}} & <1                   & 534              & 577              & 663              & 1011              & 29204               & 29183               \\ \hline
% \multicolumn{1}{l|}{\textbf{PitsC}} & <1                   & 148              & 202              & 267              & 369               & 9909                & 9898                \\ \hline
% \multicolumn{1}{l|}{\textbf{PitsD}} & <1                   & 101              & 127              & 164              & 253               & 7009                & 6914                \\ \hline
% \multicolumn{1}{l|}{\textbf{PitsE}} & <1                   & 318              & 343              & 414              & 587               & 23163               & 23154               \\ \hline
% \multicolumn{1}{l|}{\textbf{PitsF}} & <1                   & 406              & 456              & 551              & 777               & 27008               & 26927               \\ \hline
% \end{tabular}
% \end{table*}



\subsection*{\textbf{RQ2:  {\em How does simpler method perform and be explainable against recent state of the art search based SE method?} }}

Recently researchers have moved towards hyperparameter optimization to achieve better performance but they do come with an expense of heavy runtime~\cite{fu2016tuning,ghotra2015revisiting,agrawal2018wrong,agrawal2018better}. Agrawal et al.~\cite{agrawal2018wrong} showed LDADE to achieve better performance in classification task with SVM as a classifier. LDADE chooses optimal $K$, $\alpha$ and $\beta$, but $K$ matters the most for supervised learning. In this research question, we compared LDADE+SVM, LDADE+FFT against LDA+FFT. We tried multiple combinations of LDA features like ($K=10, 25, 50, 100$) with its other default values.

Figure~\ref{fig:rq1} shows the comparison between LDADE+SVM, LDADE+FFT against 10\_FFT, 25\_FFT, 50\_FFT, 100\_FFT which denotes for different K values. X-axis in the figure represents different datasets and Y-axis represents precision and recall scores.

For recall, we can observe that 10\_FFT, 25\_FFT, 50\_FFT, 100\_FFT are performing statistically similar against all 6 datasets. But they are statistically winning against LDADE+SVM on 2 out of 6 datasets, and are statistically similar on the remaining 4 occasions. LDADE+FFT is performing statistically similar against 10\_FFT, 25\_FFT, 50\_FFT, 100\_FFT. This tells that FFT is a great alternative classifier.
%Since all K values are performing similarly, we can choose $K=10$ as the optimal number of features that are needed.

For precision, a similar trend was observed where 10\_FFT, 25\_FFT, 50\_FFT, 100\_FFT are performing statistically similar but they are winning statistically on all 6 datasets against LDADE+SVM and LDADE+FFT. Though we can choose $K=10$ as the optimal number of features that are needed since all K values are performing similarly.

With any empirical study, we have to look at the runtimes to make sure they do not come at a cost of big runtime. Table~\ref{tbl:runtimes} shows the runtimes in minutes. From the table, it can be observed that LDA+FFT combination is about 500 times slower than LDADE+SVM and LDADE+FFT. This tells us that hyper optimization is quite expensive and we should look for alternative solutions which are fast. With this, FFT looks to be a promising candidate. 
\fi 

Since each term occurring in the documents is considered
an additional dimension, textual data can be of a very high
dimensionality. Introducing preprocessing steps reduce the number of considered
terms and also these terms are less informative. The typical preprocessing steps which we employed are the following:
\bi
\item \textit{Tokenization}: The process of tokenization consists of
dividing a large textual string into a set of tokens
where a single token corresponds to a single term. This
step also includes filtering out all meaningless symbols
like punctuations and commas, because these symbols
do not contribute to the classification task. Also, all
uppercase characters are replaced by their lowercase
ones.

\item \textit{Stop-words removal}: Human languages commonly
make use of constructive terms like conjunctions, adverbs,
prepositions and other language structures to
build up sentences. Terms like ``the'', ``in'' and ``that''
also known as stop-words that do not carry much specific
information in the context of a bug report. Moreover,
these terms appear frequently in the descriptions of
the bug reports and thus increase the dimensionality of
the data which in turn could decrease the performance
of classification algorithms. Therefore, all
stop-words are removed from the set of tokens based
on a list of known stop-words available from NLTK toolkit\footnote{\url{http://www.nltk.org/book/ch02.html}}~\cite{bird2006nltk}.

\item \textit{Stemming}: The stemming step aims at reducing each
term appearing in the descriptions into its basic form.
Each single term can be expressed in different forms
but still carry the same specific information. For example,
the terms ``computerized'', ``computerize'' and
``computation'' all share the same morphological base:
``computer''. A stemming algorithm like the porter
stemmer~\cite{Porter1980} transforms each term to its basic form.

\ei

==> figs/skresults.tex <==

\newcommand{\nm}[1] { \hline &\multicolumn{1}{l}{  {\bf #1 }}}


\newcommand{\ofr} {
{\textit{out-of-range}}
}
%\newcommand{\quart}[4]{\begin{picture}(100,3)%1
%{\color{black}\put(#3,3){\circle*{4}}\put(#1,3){\line(1,0){#2}}}\end{picture}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%Latex Table%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[!t]
\begin{center}

\resizebox{0.49\textwidth}{!}{\begin{minipage}{5in}
{\small
\begin{center}a. \% PRECISION  ({\em larger} values are {\em better}).\end{center}

\begin{tabular}{llrrc} 

{\textbf{Rank}}& \textbf{Using} & \textbf{Med.} & \textbf{IQR} & \\
\nm{pitsA}\\ 
    1 &      TFIDF\_SVM &    68 &  5 & \quart{66}{5}{68}{100} \\ 
    2 &      25\_FFT &    50 &  11 & \quart{48}{11}{50}{100} \\ 
    2 &      10\_FFT &    50 &  8 & \quart{44}{8}{50}{100} \\ 
    2 &      50\_FFT &    50 &  7 & \quart{47}{7}{50}{100} \\ 
    2 &      100\_FFT &    49 &  8 & \quart{44}{8}{49}{100} \\ 
    3 &      LDADE\_FFT &    40 &  13 & \quart{33}{13}{40}{100} \\ 
    3 &      LDADE\_SVM &    11 &  50 & \quart{0}{50}{11}{100} \\ 

\nm{pitsB}\\ 
    1 &      TFIDF\_SVM &    100 &  0 & \quart{100}{0}{100}{100} \\ 
    2 &      50\_FFT &    72 &  5 & \quart{69}{5}{72}{100} \\ 
    2 &      100\_FFT &    71 &  4 & \quart{69}{4}{71}{100} \\ 
    2 &      25\_FFT &    71 &  2 & \quart{70}{2}{71}{100} \\ 
    2 &      10\_FFT &    71 &  2 & \quart{70}{2}{71}{100} \\ 
    3 &      LDADE\_FFT &    39 &  11 & \quart{33}{11}{39}{100} \\ 
    3 &      LDADE\_SVM &    0 &  50 & \quart{0}{50}{0}{100} \\ 

\nm{pitsC}\\ 
    1 &      TFIDF\_SVM &    94 &  6 & \quart{91}{6}{94}{100} \\ 
    2 &      10\_FFT &    80 &  31 & \quart{69}{31}{80}{100} \\ 
    3 &      25\_FFT &    67 &  23 & \quart{60}{23}{67}{100} \\ 
    3 &      50\_FFT &    67 &  21 & \quart{50}{21}{67}{100} \\ 
    4 &      LDADE\_SVM &    56 &  1 & \quart{55}{1}{56}{100} \\ 
    4 &      LDADE\_FFT &    50 &  27 & \quart{33}{27}{50}{100} \\ 
    4 &      100\_FFT &    50 &  23 & \quart{44}{23}{50}{100} \\ 

\nm{pitsD}\\ 
    1 &      LDADE\_FFT &    100 &  12 & \quart{88}{12}{100}{100} \\ 
    1 &      100\_FFT &    100 &  6 & \quart{94}{6}{100}{100} \\ 
    1 &      10\_FFT &    100 &  4 & \quart{96}{4}{100}{100} \\ 
    1 &      50\_FFT &    100 &  6 & \quart{94}{6}{100}{100} \\ 
    1 &      TFIDF\_SVM &    97 &  3 & \quart{94}{3}{97}{100} \\ 
    1 &      25\_FFT &    94 &  8 & \quart{92}{8}{94}{100} \\ 
    2 &      LDADE\_SVM &    92 &  0 & \quart{92}{0}{92}{100} \\ 

\nm{pitsE}\\ 
    1 &      TFIDF\_SVM &    78 &  4 & \quart{75}{4}{78}{100} \\ 
    1 &      10\_FFT &    71 &  22 & \quart{64}{22}{71}{100} \\ 
    2 &      25\_FFT &    69 &  9 & \quart{66}{9}{69}{100} \\ 
    2 &      100\_FFT &    68 &  6 & \quart{64}{6}{68}{100} \\ 
    2 &      50\_FFT &    68 &  8 & \quart{64}{8}{68}{100} \\ 
    2 &      LDADE\_FFT &    67 &  13 & \quart{57}{13}{67}{100} \\ 
    3 &      LDADE\_SVM &    63 &  1 & \quart{62}{1}{63}{100} \\ 

\nm{pitsF}\\ 
    1 &      25\_FFT &    85 &  7 & \quart{80}{7}{85}{100} \\ 
    1 &      10\_FFT &    85 &  5 & \quart{82}{5}{85}{100} \\ 
    1 &      100\_FFT &    83 &  7 & \quart{81}{7}{83}{100} \\ 
    1 &      50\_FFT &    83 &  7 & \quart{81}{7}{83}{100} \\ 
    1 &      TFIDF\_SVM &    82 &  4 & \quart{80}{4}{82}{100} \\ 
    2 &      LDADE\_SVM &    64 &  0 & \quart{64}{0}{64}{100} \\ 
    2 &      LDADE\_FFT &    63 &  11 & \quart{59}{11}{63}{100} \\ 

\end{tabular}} 

\end{minipage}} 
\hspace{1mm}

\resizebox{0.49\textwidth}{!}{\begin{minipage}{5in}
{\small
\begin{center}b. \% RECALL ({\em larger} values are {\em better})\end{center}

\begin{tabular}{llrrc} 

{\textbf{Rank}}& \textbf{Using} & \textbf{Med.} & \textbf{IQR} & \\
\nm{pitsA}\\ 
    1 &      LDADE\_FFT &    95 &  4 & \quart{92}{4}{95}{100} \\ 
    1 &      10\_FFT &    95 &  4 & \quart{92}{4}{95}{100} \\ 
    1 &      25\_FFT &    93 &  3 & \quart{92}{3}{93}{100} \\ 
    1 &      100\_FFT &    93 &  4 & \quart{92}{4}{93}{100} \\ 
    1 &      50\_FFT &    93 &  4 & \quart{92}{4}{93}{100} \\ 
    2 &      TFIDF\_SVM &    71 &  8 & \quart{65}{8}{71}{100} \\ 
    3 &      LDADE\_SVM &    1 &  3 & \quart{0}{3}{1}{100} \\ 

\nm{pitsB}\\ 
    1 &      25\_FFT &    100 &  0 & \quart{100}{0}{100}{100} \\ 
    1 &      100\_FFT &    100 &  0 & \quart{100}{0}{100}{100} \\ 
    1 &      10\_FFT &    100 &  0 & \quart{100}{0}{100}{100} \\ 
    1 &      50\_FFT &    100 &  0 & \quart{100}{0}{100}{100} \\ 
    1 &      TFIDF\_SVM &    100 &  0 & \quart{100}{0}{100}{100} \\ 
    2 &      LDADE\_FFT &    95 &  2 & \quart{93}{2}{95}{100} \\ 
    3 &      LDADE\_SVM &    0 &  1 & \quart{0}{1}{0}{100} \\ 

\nm{pitsC}\\ 
    1 &      LDADE\_SVM &    94 &  21 & \quart{76}{21}{94}{100} \\ 
    1 &      LDADE\_FFT &    94 &  5 & \quart{92}{5}{94}{100} \\ 
    1 &      25\_FFT &    94 &  6 & \quart{89}{6}{94}{100} \\ 
    1 &      TFIDF\_SVM &    94 &  5 & \quart{92}{5}{94}{100} \\ 
    1 &      100\_FFT &    92 &  8 & \quart{89}{8}{92}{100} \\ 
    1 &      50\_FFT &    92 &  8 & \quart{89}{8}{92}{100} \\ 
    1 &      10\_FFT &    92 &  6 & \quart{89}{6}{92}{100} \\ 

\nm{pitsD}\\ 
    1 &      LDADE\_SVM &    100 &  0 & \quart{100}{0}{100}{100} \\ 
    2 &      TFIDF\_SVM &    97 &  3 & \quart{97}{3}{97}{100} \\ 
    3 &      LDADE\_FFT &    94 &  6 & \quart{91}{6}{94}{100} \\ 
    3 &      25\_FFT &    94 &  6 & \quart{91}{6}{94}{100} \\ 
    3 &      100\_FFT &    94 &  6 & \quart{91}{6}{94}{100} \\ 
    3 &      10\_FFT &    94 &  6 & \quart{91}{6}{94}{100} \\ 
    3 &      50\_FFT &    94 &  6 & \quart{91}{6}{94}{100} \\ 

\nm{pitsE}\\ 
    1 &      LDADE\_SVM &    100 &  1 & \quart{99}{1}{100}{100} \\ 
    2 &      25\_FFT &    95 &  4 & \quart{92}{4}{95}{100} \\ 
    2 &      100\_FFT &    95 &  2 & \quart{94}{2}{95}{100} \\ 
    2 &      10\_FFT &    95 &  4 & \quart{93}{4}{95}{100} \\ 
    2 &      50\_FFT &    95 &  2 & \quart{94}{2}{95}{100} \\ 
    2 &      LDADE\_FFT &    93 &  3 & \quart{92}{3}{93}{100} \\ 
    3 &      TFIDF\_SVM &    80 &  4 & \quart{77}{4}{80}{100} \\ 

\nm{pitsF}\\ 
    1 &      LDADE\_SVM &    100 &  3 & \quart{97}{3}{100}{100} \\ 
    2 &      LDADE\_FFT &    94 &  4 & \quart{92}{4}{94}{100} \\ 
    2 &      100\_FFT &    94 &  4 & \quart{92}{4}{94}{100} \\ 
    2 &      10\_FFT &    94 &  3 & \quart{93}{3}{94}{100} \\ 
    2 &      50\_FFT &    94 &  3 & \quart{93}{3}{94}{100} \\ 
    2 &      25\_FFT &    94 &  3 & \quart{92}{3}{94}{100} \\ 
    3 &      TFIDF\_SVM &    83 &  5 & \quart{82}{5}{83}{100} \\ 

\end{tabular}} 

\end{minipage}} 

\end{center} 

\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%End Latex Table%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> skres_temp.tex <==
\newcommand{\nm}[1]{\hline\multicolumn{1}{c}{\cellcolor{black} { {\bf \textcolor{white}{#1}}}}}

\begin{figure*}[!t]
\setlength{\belowcaptionskip}{-16pt}
\begin{center}
\renewcommand{\baselinestretch}{0.65}  
\resizebox{0.45\textwidth}{!}{\begin{minipage}{4in}
{\small
\begin{center}a. \% PRECISION  ({\em larger} values are {\em better}).\end{center}
\begin{tabular}{llrrc} 
{\textbf{Rank}}& \textbf{Using} & \textbf{Med.} & \textbf{IQR} & \\
\nm{pitsA}\\ 
    1 &      TFIDF\_SVM &    68 &  5 & \quart{66}{5}{68}{100} \\ 
    2 &      25\_FFT &    50 &  11 & \quart{48}{11}{50}{100} \\ 
    2 &      10\_FFT &    50 &  8 & \quart{44}{8}{50}{100} \\ 
    2 &      50\_FFT &    50 &  7 & \quart{47}{7}{50}{100} \\ 
    2 &      100\_FFT &    49 &  8 & \quart{44}{8}{49}{100} \\ 
    3 &      LDADE\_FFT &    40 &  13 & \quart{33}{13}{40}{100} \\ 
    3 &      LDADE\_SVM &    11 &  50 & \quart{0}{50}{11}{100} \\ 
\nm{pitsB}\\ 
    1 &      TFIDF\_SVM &    100 &  0 & \quart{100}{0}{100}{100} \\ 
    2 &      50\_FFT &    72 &  5 & \quart{69}{5}{72}{100} \\ 
    2 &      100\_FFT &    71 &  4 & \quart{69}{4}{71}{100} \\ 
    2 &      25\_FFT &    71 &  2 & \quart{70}{2}{71}{100} \\ 
    2 &      10\_FFT &    71 &  2 & \quart{70}{2}{71}{100} \\ 
    3 &      LDADE\_FFT &    39 &  11 & \quart{33}{11}{39}{100} \\ 
    3 &      LDADE\_SVM &    0 &  50 & \quart{0}{50}{0}{100} \\ 
\nm{pitsC}\\ 
    1 &      TFIDF\_SVM &    94 &  6 & \quart{91}{6}{94}{100} \\ 
    2 &      10\_FFT &    80 &  31 & \quart{69}{31}{80}{100} \\ 
    3 &      25\_FFT &    67 &  23 & \quart{60}{23}{67}{100} \\ 
    3 &      50\_FFT &    67 &  21 & \quart{50}{21}{67}{100} \\ 
    4 &      LDADE\_SVM &    56 &  1 & \quart{55}{1}{56}{100} \\ 
    4 &      LDADE\_FFT &    50 &  27 & \quart{33}{27}{50}{100} \\ 
    4 &      100\_FFT &    50 &  23 & \quart{44}{23}{50}{100} \\ 
\nm{pitsD}\\ 
    1 &      LDADE\_FFT &    100 &  12 & \quart{88}{12}{100}{100} \\ 
    1 &      100\_FFT &    100 &  6 & \quart{94}{6}{100}{100} \\ 
    1 &      10\_FFT &    100 &  4 & \quart{96}{4}{100}{100} \\ 
    1 &      50\_FFT &    100 &  6 & \quart{94}{6}{100}{100} \\ 
    1 &      TFIDF\_SVM &    97 &  3 & \quart{94}{3}{97}{100} \\ 
    1 &      25\_FFT &    94 &  8 & \quart{92}{8}{94}{100} \\ 
    2 &      LDADE\_SVM &    92 &  0 & \quart{92}{0}{92}{100} \\ 
\nm{pitsE}\\ 
    1 &      TFIDF\_SVM &    78 &  4 & \quart{75}{4}{78}{100} \\ 
    1 &      10\_FFT &    71 &  22 & \quart{64}{22}{71}{100} \\ 
    2 &      25\_FFT &    69 &  9 & \quart{66}{9}{69}{100} \\ 
    2 &      100\_FFT &    68 &  6 & \quart{64}{6}{68}{100} \\ 
    2 &      50\_FFT &    68 &  8 & \quart{64}{8}{68}{100} \\ 
    2 &      LDADE\_FFT &    67 &  13 & \quart{57}{13}{67}{100} \\ 
    3 &      LDADE\_SVM &    63 &  1 & \quart{62}{1}{63}{100} \\ 
\nm{pitsF}\\ 
    1 &      25\_FFT &    85 &  7 & \quart{80}{7}{85}{100} \\ 
    1 &      10\_FFT &    85 &  5 & \quart{82}{5}{85}{100} \\ 
    1 &      100\_FFT &    83 &  7 & \quart{81}{7}{83}{100} \\ 
    1 &      50\_FFT &    83 &  7 & \quart{81}{7}{83}{100} \\ 
    1 &      TFIDF\_SVM &    82 &  4 & \quart{80}{4}{82}{100} \\ 
    2 &      LDADE\_SVM &    64 &  0 & \quart{64}{0}{64}{100} \\ 
    2 &      LDADE\_FFT &    63 &  11 & \quart{59}{11}{63}{100} \\ 
\end{tabular}} 
\end{minipage}} 
\hspace{1mm}
%%%%%%%%%%%%%%%%%%%%%%%End Latex Table%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%Latex Table%%%%%%%%%%%%%%%%%%%%%%%%%
\resizebox{0.45\textwidth}{!}{\begin{minipage}{4in}
{\small
\begin{center}b. \% RECALL ({\em larger} values are {\em better})\end{center}
\begin{tabular}{llrrc} 
{\textbf{Rank}}& \textbf{Using} & \textbf{Med.} & \textbf{IQR} & \\
\nm{pitsA}\\ 
    1 &      LDADE\_FFT &    95 &  4 & \quart{92}{4}{95}{100} \\ 
    1 &      10\_FFT &    95 &  4 & \quart{92}{4}{95}{100} \\ 
    1 &      25\_FFT &    93 &  3 & \quart{92}{3}{93}{100} \\ 
    1 &      100\_FFT &    93 &  4 & \quart{92}{4}{93}{100} \\ 
    1 &      50\_FFT &    93 &  4 & \quart{92}{4}{93}{100} \\ 
    2 &      TFIDF\_SVM &    71 &  8 & \quart{65}{8}{71}{100} \\ 
    3 &      LDADE\_SVM &    1 &  3 & \quart{0}{3}{1}{100} \\ 
\nm{pitsB}\\ 
    1 &      25\_FFT &    100 &  0 & \quart{100}{0}{100}{100} \\ 
    1 &      100\_FFT &    100 &  0 & \quart{100}{0}{100}{100} \\ 
    1 &      10\_FFT &    100 &  0 & \quart{100}{0}{100}{100} \\ 
    1 &      50\_FFT &    100 &  0 & \quart{100}{0}{100}{100} \\ 
    1 &      TFIDF\_SVM &    100 &  0 & \quart{100}{0}{100}{100} \\ 
    2 &      LDADE\_FFT &    95 &  2 & \quart{93}{2}{95}{100} \\ 
    3 &      LDADE\_SVM &    0 &  1 & \quart{0}{1}{0}{100} \\ 
\nm{pitsC}\\ 
    1 &      LDADE\_SVM &    94 &  21 & \quart{76}{21}{94}{100} \\ 
    1 &      LDADE\_FFT &    94 &  5 & \quart{92}{5}{94}{100} \\ 
    1 &      25\_FFT &    94 &  6 & \quart{89}{6}{94}{100} \\ 
    1 &      TFIDF\_SVM &    94 &  5 & \quart{92}{5}{94}{100} \\ 
    1 &      100\_FFT &    92 &  8 & \quart{89}{8}{92}{100} \\ 
    1 &      50\_FFT &    92 &  8 & \quart{89}{8}{92}{100} \\ 
    1 &      10\_FFT &    92 &  6 & \quart{89}{6}{92}{100} \\ 
\nm{pitsD}\\ 
    1 &      LDADE\_SVM &    100 &  0 & \quart{100}{0}{100}{100} \\ 
    2 &      TFIDF\_SVM &    97 &  3 & \quart{97}{3}{97}{100} \\ 
    3 &      LDADE\_FFT &    94 &  6 & \quart{91}{6}{94}{100} \\ 
    3 &      25\_FFT &    94 &  6 & \quart{91}{6}{94}{100} \\ 
    3 &      100\_FFT &    94 &  6 & \quart{91}{6}{94}{100} \\ 
    3 &      10\_FFT &    94 &  6 & \quart{91}{6}{94}{100} \\ 
    3 &      50\_FFT &    94 &  6 & \quart{91}{6}{94}{100} \\ 
\nm{pitsE}\\ 
    1 &      LDADE\_SVM &    100 &  1 & \quart{99}{1}{100}{100} \\ 
    2 &      25\_FFT &    95 &  4 & \quart{92}{4}{95}{100} \\ 
    2 &      100\_FFT &    95 &  2 & \quart{94}{2}{95}{100} \\ 
    2 &      10\_FFT &    95 &  4 & \quart{93}{4}{95}{100} \\ 
    2 &      50\_FFT &    95 &  2 & \quart{94}{2}{95}{100} \\ 
    2 &      LDADE\_FFT &    93 &  3 & \quart{92}{3}{93}{100} \\ 
    3 &      TFIDF\_SVM &    80 &  4 & \quart{77}{4}{80}{100} \\ 
\nm{pitsF}\\ 
    1 &      LDADE\_SVM &    100 &  3 & \quart{97}{3}{100}{100} \\ 
    2 &      LDADE\_FFT &    94 &  4 & \quart{92}{4}{94}{100} \\ 
    2 &      100\_FFT &    94 &  4 & \quart{92}{4}{94}{100} \\ 
    2 &      10\_FFT &    94 &  3 & \quart{93}{3}{94}{100} \\ 
    2 &      50\_FFT &    94 &  3 & \quart{93}{3}{94}{100} \\ 
    2 &      25\_FFT &    94 &  3 & \quart{92}{3}{94}{100} \\ 
    3 &      TFIDF\_SVM &    83 &  5 & \quart{82}{5}{83}{100} \\ 
\end{tabular}} 
\end{minipage}} 
\end{center} 
\end{figure*}
